ReasVQA: Advancing VideoQA with Imperfect Reasoning Process

Video Question Answering (VideoQA) is a challenging task that requires understanding complex visual and temporal relationships within videos to answer questions accurately. In this work, we introduce \textbf{ReasVQA} (Reasoning-enhanced Video Question Answering), a novel approach that leverages reasoning processes generated by Multimodal Large Language Models (MLLMs) to improve the performance of VideoQA models. Our approach consists of three phases: reasoning generation, reasoning refinement, and learning from reasoning. First, we generate detailed reasoning processes using additional MLLMs, and second refine them via a filtering step to ensure data quality. Finally, we use the reasoning data, which might be in an imperfect form, to guide the VideoQA model via multi-task learning, on how to interpret and answer questions based on a given video. We evaluate ReasVQA on three popular benchmarks, and our results establish new state-of-the-art performance with significant improvements of +2.9 on NExT-QA, +7.3 on STAR, and +5.9 on IntentQA. Our findings demonstrate the supervising benefits of integrating reasoning processes into VideoQA. Further studies validate each component of our method, also with different backbones and MLLMs, and again highlight the advantages of this simple but effective method. We offer a new perspective on enhancing VideoQA performance by utilizing advanced reasoning techniques, setting a new benchmark in this research field.

==> 1_fig/data_efficiency.tex <==


\begin{figure}[!thb]
    \centering
    \begin{subfigure}[b]{0.236\textwidth}
        \centering
        \includegraphics[width=\textwidth]{0_pic/data_eff_nextqa_v2_separate_legends.pdf} % 替换为你的图片路径
        \caption{NExT-QA}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.236\textwidth}
        \centering
        \includegraphics[width=\textwidth]{0_pic/data_eff_star_v2_separate_legends.pdf} % 替换为你的图片路径
        \caption{STAR}
        \label{fig:sub2}
    \end{subfigure}
    \caption{The impact of data quantity on model performance and the comparison after data cleaning and filtering. All experiments are conducted using a multi-task learning approach, with both \(\alpha\) and \(\beta\) set to 0.5.}
    \label{fig:data_effect}
\end{figure}

==> 1_fig/hy_paras_onefig.tex <==
\begin{figure}[!htb]
    \centering
    % \includegraphics[scale=0.41]{0_pictures/example-test11.pdf}
    \includegraphics[scale=0.5]{0_pic/hype.pdf}
    \caption{Case study of our \model using 8 Frames on STAR.}
    \label{fig:example}
    % \vspace{-4mm}

\end{figure}

==> 1_fig/hy_paras_twofig.tex <==
% \begin{figure}[thb]
%     \centering
%     \begin{subfigure}[b]{0.231\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{0_pic/hype_nextqa.pdf} % 替换为你的图片路径
%         \caption{NExT-QA}
%         \label{fig:sub1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2211\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{0_pic/hype_star.pdf}
%         % 替换为你的图片路径
%         \caption{STAR}
%         \label{fig:sub2}
%     \end{subfigure}
%     \caption{Hyper-parameter Tuning for the weight (\(\beta\)) of the Reasoning loss, with the corresponding \(\alpha = 1 - \beta\).}
%     \label{fig:hyper_beta}
% \end{figure}



  \begin{figure}[thb]
    \centering
    \begin{minipage}[t]{0.49\linewidth} 
    \centering
    \subfigure[NExT-QA]{
    \includegraphics[width=\textwidth]{0_pic/hype_nextqa.pdf}}
        
    \end{minipage}
    % \hfill
    \begin{minipage}[t]{0.47\linewidth} 
        \centering
    \subfigure[STAR]{
    \includegraphics[width=\textwidth]{0_pic/hype_star.pdf}}
        
    \end{minipage}
        
    \caption{Hyper-parameter Tuning for the weight (\(\beta\)) of the Reasoning loss, with the corresponding \(\alpha = 1 - \beta\).}
    \label{fig:hyper_beta}
\end{figure}

==> 2_tab/ablation_loss.tex <==
\begin{table}[!thb]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|c}
\toprule
\multirow{2}{*}{Setting}  

&\multirow{2}{*}{\textbf{NExT-QA}}  &\multirow{2}{*}{\textbf{STAR}}  &\multirow{2}{*}{\textbf{IntentQA}}
&\multirow{2}{*}{\textbf{Avg.\ $\uparrow$}}\\
& & &
\\ 
 
 \midrule

STL$_{QA}$ &75.4  &71.0  &73.3  &73.2  \\
\midrule
STL$_{CR}$&74.2  &71.9  &74.4 &73.5  \\
STL$_{All}$  &73.3  &70.6  &70.8  &71.6 \\
MTL$_{CR}$ &76.2  &72.9  &76.1  & 75.1 \\
MTL$_{All}$ &76.8  &73.2  &77.0  & 75.7 \\

\midrule

\end{tabular}
}
\caption{Influence of Different Training Approaches of \model.}
\label{tb:mt_learning}
\end{table}

==> 2_tab/data_efficiency.tex <==
\begin{table}[!tb]
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
% \multirow{2}{*}{\#Frames $k_{\alpha}$} & 
\multicolumn{1}{c|}{\#Frames} & 
\multicolumn{5}{c}{\textbf{STAR}} \\
$k$&\textbf{Int.}  &\textbf{Seq.}  &\textbf{Pre.}  &\textbf{Fea.}  &\textbf{Tot.}  \\ 
 \midrule
 
 % \multicolumn{6}{c}{random } \\
 \midrule
\rowcolor{gray!5}32$\xrightarrow{}$4 &62.3  &64.7  &57.4  &54.9  &62.6    \\
\rowcolor{gray!30} 32$\xrightarrow{}$8 &68.4  &70.4  &60.9  &59.4  &68.1    \\
\rowcolor{gray!20}32$\xrightarrow{}$12 &67.2  &70.6  &62.3  &61.0  &68.0   \\
% 32$\xrightarrow{}$12 &-    &    \\
% 32$\xrightarrow{}$14 &-    &    \\
\rowcolor{gray!10}32$\xrightarrow{}$16 &65.3  &71.5  &63.0  &59.4  &67.8    \\

\midrule


\end{tabular}
% }
\caption{Comparison of model performance across different \( k \) frames (\( k = \{4, 8, 12, 16\} \)) in training. We use the same number of frames for evaluation as well as for training.
% Ablation on the number of selected frames when using the same number of frames for both training and inference on STAR.
}
% - indicates the non-use of that component.} 
\label{tb: numframes}
%
% \vspace{-3mm}
\end{table}




==> 2_tab/llava7B.tex <==
\begin{table}[!thb]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|lll}
\toprule
\multirow{2}{*}{Setting}  

&\multirow{2}{*}{\textbf{NExT-QA}}  &\multirow{2}{*}{\textbf{STAR}}  &\multirow{2}{*}{\textbf{IntentQA}}  \\
\\ 
 
 \midrule



% \color{red}Single-Task$_{all}$  &73.3  &70.6  &70.8   \\

% Multi-Task &76.8  &73.1  &77.0    \\
llava-ov(0.5B) &64.2  &60.0  &58.9    \\

+ our Rea  &65.8(+1.6) &61.5(+1.5) &63.2(+4.3)   \\
\midrule

llava-ov(7B) &77.5  &66.2  &74.1    \\

+ our Rea  &77.9 &67.9 &77.6(+3.5)   \\
\midrule

\end{tabular}
}
\caption{Ablation study for each component of \model.}
\label{tb:llava7}
\end{table}

















